Inference-Time Policy Adapters (IPA): Tailoring Extreme-Scale LMs without Fine-tuning

While extreme-scale language models have demonstrated exceptional performance on a variety of language tasks, the degree of control over these language models through pure prompting can often be limited. Directly fine-tuning such language models can be effective for tailoring them, but it can be either extremely costly (e.g., GPT-3) or not even feasible for the broader community (e.g., GPT-4). We propose Inference-time Policy Adapters (IPA), which efficiently tailors a language model such as GPT-3 without fine-tuning it. IPA guides a large base model during decoding time through a lightweight policy adapter trained to optimize an arbitrary user objective with reinforcement learning. On five challenging text generation tasks, such as toxicity reduction and lexically constrained generation, IPA consistently brings significant improvements over off-the-shelf language models. It outperforms competitive baseline methods, sometimes even including expensive fine-tuning. In particular, tailoring GPT-2 with IPA can outperform GPT-3, while tailoring GPT-3 with IPA brings a major performance boost over GPT-3 (and sometimes even over GPT-4). Our promising results highlight the potential of IPA as a lightweight alternative to tailoring extreme-scale language models.

==> sections/0_abstract.tex <==
\begin{abstract}
%Extreme-size general-purpose language models have taken the center stage of NLP field. Despite their impressive performance, language models still suffer from critical failures and cannot fulfill user requests. For instance, GPT-3's success rate in constrained generation with ordered lexical constraint is markedly low at only 29 percent. Due to the extreme size and limited access 

%, including the inability to satisfy hard logical constraints, generate faithful responses grounded in given knowledge, and avoid producing undesirable content based on non-Western values.

%Despite their impressive performance, language models still suffer from a range of critical failures, such as inability to satisfy hard logical constraints, generate faithful reponse grounded on given knowledge, or to avoid generating undesirable content based on non-Western values.
%Extreme-size language models have taken the center stage of NLP field.
%Despite their exceptional performance and capabilities of following instructions, the degree of the control over these language models through pure prompting can often be limiting. 
 While extreme-scale language models have demonstrated exceptional performance on a variety of language tasks, the degree of control over these language models through pure prompting can often be limited.
Directly %fine- \peter{removed 'fine-' because I think this is often more associated with supervised learning. But we can add it back}
tuning 
such language models can be effective for tailoring them, but it can be either extremely costly (e.g., GPT-3) or not even % available as an option
feasible for the broader community (e.g., GPT-4).

%Extreme-size language models have taken the center stage of NLP field with their exceptional performance.
%\qin{We may remove the first sentence}
%While the capabilities of following instructions allow for a convenient way to control the output of these large language models, the degree of the control can often be limiting. Directly fine-tuning such language models can be effective for tailoring them, but it can be either extremely costly (e.g., GPT-3) or not even % available as an option
%feasible for the broader community (e.g., GPT-4). \
% \sean{perhaps 'infeasible due to cost or access restrictions (e.g. GPT-3).(one could argue that extreme cost is a type of infeasibility, i.e. fine-tuning is infeasible given a particular budget)} \peter{Agree. Also, could be worth highlighting that finetuning these models is outside of our control. OpenAI could revoke this, or limit it etc. So we need methods that work off of the new model of API access}
%\liwei{IPA doens't apply to gpt4 too as they don't even have logits publically available. Probably want to be more careful about mentioning gpt4}. \jaehun{Direct fine-tuning is one way to tailor these models, but could be extremely costly if not infeasible (e.g. with GPT-4).}
%Moreover, for some applications (e.g. detoxification), it may be infeasible or even impossible to collect the necessary data for fine-tuning. \yejin{do we really need to say this previous sentence here? the problem i see is that it invokes users why not RLHF? and we don't want to trigger that thought of questions here...}
%
%\yejin{true, but I worry that trying to be super precise about it introduces other problems (e.g., the community not realizing the issue to their heart enough --- because surprisingly common mindset people have seems to be just to rely on GPT-X APIs) and i want to clearly remind what is not available }
In this paper, we propose an alternative approach, \textbf{Inference-time Policy Adapters (\beer IPA)}, that can efficiently tailor a target language model such as GPT-3 without fine-tuning it.
%
%Large language models (LLMs) like ChatGPT, often struggle to generate text aligned with users' needs, such as faithfulness, safety, coherence and more. Traditional methods for addressing this issue involve expensive fine-tuning, while recent inference-time control methods are task-specific or rely on costly gradient computation. In this paper, we introduce Reinforced Decoding (\mtd), an efficient and flexible approach for generating user-aligned, high-quality text without LLM training. 
%
%\ipa guides a large base model (such as GPT-3) during decoding by training a lightweight policy adaptor to reflect any arbitrary user objective with reinforcement learning.  
\ipa guides a large base model (such as GPT-3) during 
decoding time through a lightweight policy adapter trained to reflect any arbitrary user objective with reinforcement learning. 

Experimental results on five challenging text generation tasks, such as toxicity reduction, lexically constrained generation, open-domain generation, demonstrate that \ipa consistently brings significant improvement over off-the-shelf language models, outperforming competitive baseline methods --- sometimes even including expensive fine-tuning. In particular, we find that tailoring GPT-2 with \ipa can outperform GPT-3, while tailoring GPT-3 with \ipa brings a major performance boost over GPT-3 (and sometimes even over GPT-4). 
%Our promising results highlight the potential of \ipa to improve LLM alignment in a cost-effective and adaptable manner.
%
Our promising results highlight the potential of \ipa as a lightweight alternative to %aligning%\lasha{steering instead of aligning?}\fb{tailoring to match title?} 
tailoring extreme-scale language models.
\end{abstract}

==> sections/1_introduction.tex <==
\section{Introduction}


%\fb{Faeze: Feel free to comment/edit}
% \nouha{going over this now}
Large language models (LLMs) have recently shown remarkable progress in various text generation tasks by adapting to human instructions~\citep{ouyang2022training, gpt-3}.
% (controllable)
%or a few in-context examples~\citep{gpt-3}.  
However, the degree of control (e.g., the inclusion of keywords, avoiding harmful language) offered by these extreme-scale models
%in zero/few-shot settings 
through pure prompting is still limited~\cite{Lou2023IsPA, Webson2021DoPM}. %\qin{We may give some examples for "control", so readers know what we mean by "control" specifically. e.g. "Lexically constrained generation is to ensure inclusion of keywords in output."} 
Moreover, previous studies have found that prompting can be a brittle process due to LLMs being overly sensitive to the surface-form of the instructions \cite{perez2021true,lu-etal-2022-fantastically}. Furthermore, even with a carefully written prompt, LLMs may still struggle to fulfill certain task requirements due to their inherent limitations~\cite{liu2022tokenlevel, zong2022survey}.

\begin{figure}
    \centering
    \includegraphics[width=0.5\textwidth]{figures/fig1.pdf}
    %\caption{\peter{Completely redesigning fig1, but here is the first, stand-in draft}\fb{peter can we include "Target Model" somewhere. We can also include a snow (freezing) emoji/icon next to frozen parameters?}}
    \caption{Inference-time Policy Adapters (IPAs) efficiently steer a large-scale language model (such as GPT-3) during decoding time through a lightweight policy adapter trained to reflect any arbitrary user objective with reinforcement learning.}
    \label{fig:intro_fig}
\end{figure}

Resource-intensive fine-tuning, through supervised learning, and more recently reinforcement learning (RL) \cite{DBLP:journals/corr/abs-2205-13636} have shown promise in aligning language models to arbitrary user-specified objectives%user-specific preferences% (e.g., inclusion of keywords, being non-toxic etc.)
. However, they can be computationally expensive if not outright infeasible~\cite{OpenAI}. This issue is even more severe when access to the model's parameters (e.g., GPT-4) or powerful computational resources is restricted. 
%fine-tuning LLMs to specific tasks or domains can be computationally expensive and even infeasible~\cite{}, especially when access to the model's parameters (e.g., GPT-4) or powerful computational resources is restricted. 
% \qin{We may want to follow the flow in abstract: in-context learning paradigm, fine-tuning paradigm -> our paradigm. I feel like this paragraph about RL in between seems a little bit distractive. We may shorten this paragraph?}\fb{We didn't talk about RL in the abstract but I felt it is necessary due to the fact that we are leveraging the complementary advantages of both RL and inference-time algorithm. } Recently, Reinforcement Learning (RL)~\citep{} has emerged as a promising paradigm to align language models %outputs to user-specific preferences 
% to arbitrary objectives through reward optimization. Despite being notoriously difficult to train and highly sensitive to variance in the reward function~\citep{}, directly applying RL methods to LLMs can be computationally costly due to the need for updating all model parameters. To address the stability issue, \citet{DBLP:journals/corr/abs-2205-13636} proposed an algorithm to optimize token-level rewards that quantifies an (un)wanted property while maintaining proximity to the original language model through KL-divergence penalty.
On the other hand, \textit{inference}-time algorithms offer an efficient alternative to tailor the output of LLMs. These algorithms align language models' outputs with desired task/user-specific properties 
%such as safety, logical coherence, faithfulness, etc, 
by perturbing LM's output distribution based on certain task-specific heuristics, while leaving the underlying LMs untouched. Despite the progress, these approaches are either restricted to specific tasks \cite{DBLP:conf/naacl/LuWZBBC21, lu2020neurologic}, require domain-specific knowledge \cite{DBLP:conf/acl/LiuSLSBSC20, Yang_2021}, suffer from expensive run-time at inference \cite{qin2022cold, qin2021future, dathathri2020plug}, or have shown to be less effective compared to direct RL optimization \cite{DBLP:journals/corr/abs-2205-13636}.



%\textit{Inference}-time algorithm offers a compelling alternative for expensive fine-tuning. These algorithms can adapt language models outputs to task/user-specific properties such as safety, logical coherence, faithfulness, etc. through ensembling output distributions of specialized experts~\cite{DBLP:conf/acl/LiuSLSBSC20,yang-klein-2021-fudge}, or applying gradient updates to hidden states from attribute classifiers~\cite{DBLP:conf/iclr/DathathriMLHFMY20}. More recent approaches use energy-based modeling for incorporating constraints \cite{DBLP:journals/corr/abs-2202-11705, DBLP:journals/corr/abs-2203-13299}. Despite the progress, these approaches either focus on specific tasks or rely on computationally expensive gradient calculations.

%\liwei{Beyond efficiency and generalizability, it would be nice to highlight the \method has the critical advantage of being able to maintain the good qualities of the base policy model while using the adapter module to encode the desired quality. The previous RL paradigm that operates directly on the base policy parameter risks overfitting to the reward and thus losing already existing good properties of the base policy.} \ximing{not sure this apply, since in IPA framework any RL algorithm can be used, whether overfitting to the reward on not depends on the RL we chose to plug in}
\liwei{at a high level, it might be good to spend a few sentences to explicitly spell out the advantages of \method---right now it feels we are being too humble in selling the advantage of the method. For example, efficiency, generalizability, on-target accomodation of the specified goal, flexibility, transferable, reusuable} 
Drawing inspiration from RL and inference-time techniques,
we propose \textbf{Inference-time Policy Adapters (\beer IPA)}, a novel algorithm that is both generalizable and efficient. 
\yuchen{can we rephrase this important sentence to be a bit more specific such as ``we propose \textbf{Inference-time Policy Adapters (\beer IPA)}, a generalizable, efficient algorithm for \textit{tailoring LLMs} (or xxx). ''}
% in adapting models to arbitrary goals} leverages the benefits of both. % RL and inference-time techniques. 
IPA can efficiently tailor a target LM (such as GPT-3) during decoding time toward arbitrary task-specific objective(s) without the need to fine-tune it. 
To achieve this, we combine the output distribution of the target model with that of a smaller-size model (\textbf{policy adapter}) and optimize the combined distribution with an RL algorithm to maximize the given objective(s). During RL training, we keep the parameters of the target LM frozen and solely update the parameters of the adapter. 
%In situations where the target model is extremely expensive (such as GPT-3), we utilize a proxy model to approximate the target model's distribution for the RL training, which can either be a smaller model from the same language model family or a distilled version of the target model. 
In situations where the target model is extremely expensive (such as GPT-3), we utilize an \textbf{approximate policy}, a smaller proxy model that approximates the target model's distribution, during the RL training. The approximate policy can either be a smaller model from the same language model family or a distilled version of the target model.
At inference time, we decode with the combined distribution of the target model and the trained policy adapter.

Extensive experiments across six challenging text generation tasks demonstrate that \ipa consistently brings significant improvements over off-the-shelf language models, outperforming competitive baselines --- sometimes even including expensive fine-tuning. In particular, we find that tailoring GPT-2 with \ipa can outperform GPT-3, while tailoring GPT-3 with \ipa brings a major performance boost over GPT-3 (and sometimes even over GPT-4). 
Our compelling results highlight the promise of \ipa as a lightweight alternative for tailoring extreme-scale language models, showcasing its potential as an efficient tool for the NLP community to augment or customize LLMs without industry-level resources.%using only academic-level resources. \peter{Wondering if we have to be careful here -- it's possible that not all academic groups can afford sufficient calls to GPT-3 even for this}

%It achieves this by combining the distribution of the target model with that of a small-size model (policy adapter) and optimizing the combined distribution towards maximizing the given objective(s) through RL framework.


%during exploration and only updating the adapter policy in an RL framework [or: ... and deploying an RL framework to solely update the policy adapter]. The advantage of our method is three-fold: \fb{Talk about efficiency, generalization, modality}....

% by updating a small language model (policy adapter) while freezing the parameters of a (large) target model.



% In this paper, we propose Reinforced Decoding (RD), an efficient and flexible decoding approach using RL to generate user-aligned, high-quality text. Instead of expensive training on large-scale models (e.g., GPT-3), we train a small value model (e.g., based on GPT-2) to guide the large model's generation for value alignment. The smaller value model allows efficient use of RL in learning user preferences. Specifically, we obtain the value model by first distilling from the large base model and then fine-tuning through RL with desired reward functions such as safety, coherence, constraint satisfaction, etc. 
% %The resulting value model effectively captures user preferences, leading to improved generation quality. 
% Our method then combines the small value model with large base models to steer generations on the fly, producing fluent text aligned with users' needs.

% Through evaluations on different language generation tasks across diverse domains, including soft- and hard-constraint generation, open-ended generation, and dialogue generation,  RD consistently outperforms various baseline methods, showcasing its effectiveness in achieving user-aligned text generation. 


\begin{comment}
    

\ximing{I'll work on method first}
\ximing{skeleton of new version, WIP}

Large-scale language models (LMs) have taken the center stage of NLP field with their exceptional performance. They have shown remarkable progress for various text generation tasks \cite{}, and their instructional following ability make it easy for user to use out-of-the-box.

While these LMs are has the capability to follow instructions, users have a limited degree of the control over those language models by pure prompting...\ximing{cite} Previous studies have indicated that prompting is a brittle process, where even small modifications can lead to significant variations in generation. Additionally, models may struggle to fulfill the task request, despite our efforts to carefully structure the prompt, due to inherent limitations. \ximing{cite}

Recent works have demonstrated that reinforcement learning (RL) is an effective approach of aligning language models with an arbitrary objective post-hoc across diverse settings, such as unlearning toxicity \cite{Lu2022QuarkCT}, controlling sentiment \cite{Lu2022QuarkCT, Ramamurthy2022IsRL}, or improving human preference \cite{stiennon2022learning}.

%language model fail the understand or follow the prompts in many cases, and prompting is brittle wherein small modifications can cause large variations in generation.






\liwei{following is generated by gpt4 based on the outline below lolllll}


Extreme size Language Models (LLMs) have recently taken center stage in the field of language technology, demonstrating impressive performance across a wide range of tasks. However, they also exhibit a variety of critical failures, an issue that is well recognized within the research community. What is even more concerning is the practical impossibility of correcting or customizing these models, especially for users with limited computational resources.

This difficulty arises from several factors: most powerful and popular LLMs only provide "white-box" settings via API calls, meaning that users only have access to output logits without full access to model parameters; fine-tuning of large models is incredibly costly and cumbersome; and fine-tuning may not be the best approach to fix all issues of models, as it can lead to overfitting and loss of desirable properties.  Reinforcement Learning for Human Feedback (RLHF) has shown great success in customizing model outputs while maintaining good language qualities, but updating all parameters of a large model is extremely inefficient, if not impossible, due to the common "white-box" setting. On the other hand, inference-time algorithms offer a more efficient alternative but are often narrowly focused and designed for specific tasks.

In this paper, we address the question: \textit{``Do we really need to update all the parameters of a model to effectively adjust its behaviors according to a specified goal? And is there a more compute-efficient and adaptable way to improve any LLMs, especially those 'white-box' models given the limited access to the model parameters?''} Our goal is to combine the complementary advantages of RL algorithms and decoding-time algorithms, specifically (1) the flexibility of RL approaches that allow aligning LLMs to arbitrary goals, and (2) decoding-time algorithms that do not require full model parameter updates and can be quickly adapted to various tasks.

To achieve this, we introduce \textit{\method}, an efficient and flexible decoding approach that utilizes Reinforcement Learning (RL) to generate user-aligned, high-quality text. At a high level, our algorithm efficiently adapts LLMs to user-specific requirements without the need for extensive parameter updates or fine-tuning, thus enabling rapid and flexible customization of model behavior.

We evaluate \method across various tasks and demonstrate its empirical effectiveness, highlighting several key advantages:

\begin{itemize}
    \item \textbf{Efficiency}: Our method significantly reduces the computational cost associated with updating model parameters, enabling more accessible adaptation of large LLMs.
    
    \item \textbf{Generalizability}: Unlike task

    -specific inference-time algorithms, \method is designed to be broadly applicable across a wide range of tasks, demonstrating robust performance in diverse settings.

    \item \textbf{Accessibility}: By circumventing the need for full access to model parameters, our approach makes it possible for users to improve "white-box" LLMs even with limited computational resources.

    \item \textbf{Customization}: \method offers a flexible framework for aligning LLMs to user-specified goals, harnessing the power of RL to drive model behavior towards desired outcomes without the pitfalls of overfitting or loss of desirable properties.
\end{itemize}

In conclusion, our work on \method presents a novel approach that combines the strengths of RL and decoding-time algorithms to provide a more efficient, generalizable, accessible, and customizable solution for improving the performance of large LLMs. By addressing the current limitations in correcting and customizing these models, we hope to pave the way for more practical and versatile applications of language technology in the future.

------

\liwei{Potential intro outline. Few qualities to highlight for our approach:

\begin{itemize}
    \item \textbf{Efficiency}: don't need to full parameters of LLMs, but only on a small \adapter to steer model during inference time (inherit from decoding-time algo)
    
    \item \textbf{Generalizability}: able to align model with any arbitrary goal (inherit from RL)
    
    \item \textbf{Accessibility}: Making updating ``white-box'' with only API access of the logits (without full access of model parameters), and massive-size models that's mostly impossible to perform direct tuning with limited compute resource, possible.
    
    \item \textbf{Customization / steerability}: tailoring the close-sourced model infrastructures, massive-size models, making the best use of these powerful, yet, imperfect models 
\end{itemize}
}

\liwei{===== beginning of the outline =====}

% \liwei{
\begin{itemize}
    \item Extreme size LLMs are currently taking the center stage of languege technology. While they are impressive, they show a variety of critical failures. (notes: we could be very brief on this point as people essentially share common stand this.) 
    
    \item Even worse than the fact that the models are imperfect is it's practically impossible to correct / customize these models nowadays, especially with limited compute resources, due to
        \begin{enumerate}
            \item the most powerful and popular LLMs only provide ``white-box'' settings via API calls, meaning that we only have access of their output logits etc. without full access to model parameters.
            \item sometimes they do provide service for finetuning the model, but fintuning of LARGE models is incredibly costly and cumbersome.
            \item Not to say that fine-tuning is not necessarily the best approach to fix all issues of models, as [a] fintuning leads to overfitting to the training data/task and the loss of desirable properties, [b] sometimes there's no supervised data (notes: could adapt some points from QUARK, but keep very brief probably)
            \item there's another line that use RL for aligning models (RLHF). This line of research has shown great success in customizing model outputs to specific properties while maintaining all good language qualities, but similarly, updating all parameter of a LARGE lm is extremely ineffective if not impossible due to the common ``white-box'' setting. \textbf{the upside is}, using RL we can essentially update models based on any arbitrary goals/feedback
            \item inference-time algorithms is an alternative line of research that attempts to do lightweight adaption of large models, but it's usually narrowly focused and designed to specific tasks. \textbf{the upside is}, it's really efficient during inference time, compared to updating all parameters of a model
        \end{enumerate}

    \item  \textbf{While the popular RLHF paradigm shows the effectiveness of RL approaches via updating the full parameters, do we really need to update all the parameters of a model to be able to really adjust it's behaviors according to a specified goal?} Is there a more compute efficient / adaptable way to improve any LLMs, especially those ``whitebox'' models given the limited access to the model parameters?
        \begin{itemize}
            \item In this paper, we aim to combine the best of both worlds of (complementary advantages of RL algos and decoding time algo) (1) the flexibility of RL approaches that allow aligning LLMs to arbitrary goal; (2) decoding-time algorithm that doesn't require full model parameter update and could plug-and-play (agility, adaptability, flexibility)
        \end{itemize}
    \item We introduce \method, an efficient and flexible decoding approach using RL to generate user-aligned, high-quality text. (introduce the algorithm at high-level)
    \item (briefly talk about tasks, empirical results, and highlight the advantages of the method)
        \begin{itemize}
        \item \textbf{Efficiency}...
        
        \item \textbf{Generalizability}...
        
        \item \textbf{Accessibility}...
        
        \item \textbf{Customization}...
    \end{itemize}
    
\end{itemize}


\liwei{===== end of the outline =====}



\qin{This is an draft. Feel free to edit.} \\
Large language models (LLMs) have made significant progress in several text generation tasks. However, ensuring that the generated text adheres to specific user preferences, such as accuracy to the input information, adherence to content safety guidelines, harmlessness, and logical consistency, continues to be a challenge. This issue, known as "alignment," is crucial to make LLM-generated content more useful and acceptable to users.
\fb{Although Large language models (LLMs) have shown remarkable progress in various text generation tasks, their accessibility through API calls can be expensive and pose reproducibility challenges. Additionally, these models may learn and perpetuate unwanted behaviors that are not in line with human users' preferences, such as violating safety guidelines, being toxic, or lacking logical consistency. It is this essential to align LLM-generated content with user-specific preferences, however; there aren't many general and efficient methods for steering text generation from these models.}




% \liwei{some of the following method details could go to related work}
Traditional methods often involve resource-intensive \emph{fine-tuning}, through either supervised or reinforcement learning (RL). In particular, RL has proven effective for injecting user preferences in LM parameters \cite{DBLP:journals/corr/abs-2205-13636}. However, RL for text generation is notoriously difficult to train and costly for large models \qin{cite}.
To reduce training costs, another line of research resorts to \emph{inference}-time control. For instance, prior work manipulates LLM output distributions by mixing with specialized expert models or applying gradients from evaluator models \cite{DBLP:conf/iclr/DathathriMLHFMY20, DBLP:conf/acl/LiuSLSBSC20}; more recent approaches use energy-based modeling for incorporating constraints \cite{DBLP:journals/corr/abs-2202-11705, DBLP:journals/corr/abs-2203-13299}. Despite progress, these approaches either focus on specific tasks or rely on computationally expensive gradient calculations.

\end{comment}


% \fb{safety, constraint satisfaction, coherence, etc.}\qin{e.g.}.
 % \fb{Our method enables combining the value model with large base models to steer the generations on the fly and produce fluent text aligned with users' needs.}



% \fb{, including soft- and hard-constraint generation, open-ended generation, and dialogue generation}\qin{e.g.}, RD consistently outperforms various baseline methods, showcasing its effectiveness in achieving user-aligned text generation. \qin{add more details here}

==> sections/2_method.tex <==

% \section{Method}
\section{Inference-time Policy Adapters (IPA)}
%\fb{Ximing, pls go over method section. I directly applied minor edits and left comments for the rest} \ximing{thanks! making a pass now}

In this section, we first describe the problem statement (\S\ref{subsec:problem}), followed by a preliminary background on reinforcement learning for LM alignments (\S\ref{subsec:RL}). We then discuss our proposed \ipa algorithm for tailoring extreme-scale LMs without fine-tuning (\S\ref{subsec:IPA}).

 % without the need for expensive fine-tuning.}
%\sout{In order to generate text that is tailored to specific user objectives, without the need for expensive fine-tuning, we introduce Inference-time Policy Adapters (IPA). IPA is a lightweight module that steers a LLM to generate text consistent with user objectives during inference (\S\ref{subsec:IPA}). 
%Through RL with appropriate reward functions, IPA effectively learns the user's objectives (\S\ref{subsec:train-IPA}). We combine IPA's predictive distribution with the LLM's distribution to steer the LLM outputs \fb{during decoding?}. Figure provides an overview \qin{better to have a detailed model figure}. }


\subsection{Problem Statement}
\label{subsec:problem}
%\fb{this is about notations/problem statement} 
Conditional Text generation is the task of generating an output sequence $\textbf{y}$ given an input sequence $\textbf{x}$.
%For the general (controllable) text generation task, we
We consider the dominant paradigm for modern LLMs, i.e., the standard, left-to-right, auto-regresssive model parameterized by $\theta$, which decomposes sequence probability into token-level probability $p_\theta(\textbf{y}|\textbf{x}) = \prod^{|\textbf{y}|}_{t=1} p_\theta(\textbf{y}_t|\textbf{y}_{<t}, \textbf{x})$.
% Text generation is the task of generating an output sequence $\textbf{y}$ given an input sequence $\textbf{x}$.
% \qin{"text generation" is actually quite general topic. I think we should directly start with controlled generation. }
%For a g
\peter{We jump into talking about rewards here, although the paragraph starts by talking about conditional generation which often just uses CE loss. Maybe mention RL here?} \fb{good point! How about removing the clause "quantified by a reward function" from here, and define that in 2.2?} \peter{thinking about this. The full second half of this subsection seems to be about reward functions}\fb{On second thought, it is making a natural connection to the next subsection, right? maybe needs some editing?}
Given a model $p_\theta$, the goal is to align $p_\theta$ with some user-specified objective, quantified by a reward function $\mathcal{R}: \mathcal{Y} \rightarrow \mathbb{R}^1$ which maps output $\textbf{y}$ to a scalar score. The reward function can be defined to reflect any desired attribute such as faithfulness, safety, politeness, or constraint satisfaction. Concretely, we aim to encourage the given model $p_\theta$ to generate sequence $\textbf{y}$ with high reward score $\mathcal{R}(\textbf{y})$ while preserving reasonable language quality (e.g., fluency, coherence, diversity).

\subsection{Preliminary: RL for LM Alignment } \label{subsec:RL}
% \qin{Should we use alignment or control? We need to use consistent term through out the paper. (In abstract we already use control.)} 
%\FB{later we might shorten the preliminary RL section}
% \qin{I agree that we could shorten this sub-section.} 
Recent studies have shown the effectiveness of using online policy-based reinforcement learning, such as PPO \cite{stiennon2022learning}, Quark \cite{Lu2022QuarkCT}, or NLPO \cite{Ramamurthy2022IsRL}, to align a given language model (referred as \textit{policy} in RL framework) with an arbitrary objective post-hoc \liwei{it's a little unclear why we mention post-hoc here, or what it means in this case}\fb{+1}.
%In RL framework, we refer to the model $p_\theta$ as a policy, a partial output $\textbf{y}_{<t}$ as a state, the selection of the next token $\textbf{y}_{t}$ as an action, and the full generation of $\textbf{y}$ as an episode.
Formally, policy-based RL algorithms optimize a given policy $p_\theta$ towards generating output $\textbf{y}$ that maximizes a given reward $\mathcal{R}$ by directly updating the parameter of $p_\theta$ through gradient ascent,
\begin{align*}
    \theta^\star = \arg\max \mathbb{E}_{\textbf{y}\sim p_\theta(\cdot | \textbf{x})}\mathcal{R}(\textbf{y})
\end{align*}

During training, the policy $p_\theta$ explores the action space by generating output $\textbf{y}$ and receiving feedback through a reward function $\mathcal{R}(\textbf{y})$, which scores the output. 
The interactive nature of online RL enables policy optimization to be conducted using only model-generated outputs, eliminating the need for collecting human-written data\fb{$\leftarrow$ we can essentially remove this sentence (remember this is just a brief background)}. \liwei{Online RL uses only model-generated outputs to optimize the policy without the need for collecting human-written data.}
%To optimize $p_\theta$ towards a high reward area, the common approach is to maximize the expected return (i.e. expected reward at the end of episode) over each state, formally $\displaystyle{\maximize_{\theta} \hat{\mathbb{E}_t}}\big[\log p_\theta(\textbf{y}_t|\textbf{y}_{<t}) \hat{A}_t\big]$, such that good actions that maximize the return are sampled more frequently in the future\fb{$\leftarrow$previous sentence is a good candidate to remove for shortening (modified next sentence already)}. While %various RL algorithms may implement the exact optimization differently
%While there are different implementations to optimize $p_\theta$ towards a high reward area, 
While various RL algorithms implement the exact optimization differently,
we view the set of online policy-based RL algorithms as a family of functions $\mathcal{F}_{\textnormal{RL}}$ that take a policy $p_\theta$ and a reward function $\mathcal{R}$ as inputs and produce an optimized policy $p_{\theta^\star}$ with respect to $\mathcal{R}$ via gradient ascent on $\theta$. Formally,
\begin{align*} 
\mathcal{F}_{\textnormal{RL}} = \{ f_{\textnormal{RL}}: (p_\theta, \mathcal{R}; \theta) \rightarrow \theta^\star \}
\end{align*}


%Inference-time Policy Adapters (IPA) go through two stage to tailor a target large-scale language model to align with user

% \subsection{Inference-time Policy Adapters (IPA)}  \label{subsec:IPA}

\subsection{Tailoring LLMs with IPA} \label{subsec:IPA}
% Despite the success of RL, it's not feasible to perform RL optimization on extreme-scale LMs like GPT-3, due to limited access and high costs.  
% Instead, we propose Inference-time Policy Adapters (IPA), 
% a lightweight module that steers a frozen target language model during decoding time to align it with arbitrary user given objective.
% Despite the success of RL in aligning LMs with a user's objectives, its application to LLMs like GPT-3 is inefficient and often infeasible \liwei{for the broader community} due to substantial computational costs and limited accessibility. 
% \FB{I'd suggest referring to a detailed figure and then start describing the components/sections.}
We propose Inference-time Policy Adapters (IPA), a lightweight module trained with reinforcement learning to steer the outputs of a frozen target LLM towards user-specific objectives, as illustrated in Figure \ref{fig:intro_fig} and detailed below.
\method is a more lightweight and effective alternative than using RL in updating all model parameters, which is inefficient and often infeasible for LLMs like GPT-3 due to substantial computational costs and limited accessibility.

% Despite the success of RL in aligning LMs with a user's objectives

\subsubsection{Policy Adaptation}
First, we will demonstrate how a policy adaptor is used to augment the output distribution of a given language model, starting with defining a few key terminologies.
\begin{definition}[base policy]
The given language model to tailor is referred as base policy.
\end{definition}
\begin{definition}[policy adapter]
The inference-time policy adapter (IPA) is defined as a neural network that is parameterized by $\phi$ and shares the same output space $p(\cdot|\textbf{y}_{<t})$ as the base policy. IPA is referred to as the policy adapter.
\end{definition}
\noindent  In practice, we initialized the policy adapter \nouha{we have to be consistent, use one of those: policy adaptor or adaptor policy} \liwei{that's a great point! to distinguish from adapted policy, maybe we should say "policy adaptor". or maybe we should reconsider the terminology "adapted policy", which is a tad confusing that it refers to base policy + adaptor. maybe we can use some more distinctive word to describe it like "tailored policy", "fused policy"} \fb{so far we have been using policy adapter everywhere (except in def 2). I think we can stick to the policy adapter and change the adapted policy -> tailored policy.} with a small language model in the same model family as the base policy to have them share the same vocabulary space. 

%\nouha{I totally agree, the adapted policy is confusing. We  should either merge it with the adaptor policy definition or  change its naming. To reduce confusion, we can include it under \ipa definition and at the end that's the contribution of \ipa: combining the distributions of a frozen policy and a trained one. }
%a smaller language model with shared vocabulary space as the base policy. 
\begin{definition}[adapted policy]
The adapted policy $p_{\theta \leftarrow \phi}$ is defined as a product of experts combining the distributions of the base policy $p_{\theta}$ and the policy adapter $p_{\phi}$, formally 
\vspace{-2.5mm}
\begin{align*} 
p_{\theta \leftarrow \phi} (\textbf{y}_{t}|\textbf{y}_{<t}) = \frac{1}{Z}  p_{\theta} (\textbf{y}_{t}|\textbf{y}_{<t}) p_{\phi}(\textbf{y}_{t}|\textbf{y}_{<t})
\end{align*}
where $Z$ is a normalization factor to ensure valid probability distribution.
\end{definition}
Our goal is to align adapted policy with the given objectives, which will be detailed in the following section.
The proposed policy adaption offers several favorable properties: Firstly, late fusion at the distributional level enables steering the given LLM without access to its model parameter, accommodating the limited accessibility of most powerful and widely used LLMs through API calls, where users only have access to output logits. 
% but not full model parameters. 
Secondly, the policy adapter can be instantiated with a much smaller model, providing an efficient approach to guide a significantly larger language model.

%We instead present Inference-time Policy Adapters (IPA), a lightweight module to steer the outputs of a frozen target LLM towards user-specific objectives. Figure \ref{fig:intro_fig} illustrates an overview of \ipa algorithm. In this method, we combine the output distribution of a target LM with that of a smaller-sized model during inference. We then employ a reinforcement learning (RL) algorithm to optimize the combined distribution, aiming to maximize the specified user objective(s) (\S\ref{subsec:train-IPA}). By training IPA with RL, we are able to take advantage of RL's strengths, while circumventing its considerable computational costs  through inference-time adaptation.
% \sout{Instead, we propose IPA, a lightweight module trained via RL to steer a frozen target LLM during inference, aligning it with any arbitrary user objective. By training IPA with RL, we're able to take advantage of RL's strengths, while simultaneously avoiding its substantial costs.}

%\qin{Describe the overall framework here.}\\
% \qin{We could first describe the overall framework before talking about the detailed implementation, like "Initialization".}\fb{+1}

% \fb{The overview of \ipa is depicted in Figure \ref{} which consists of ...}

% \paragraph{Adapting Target Policy.}
% \FB{changed initialization. Still open to suggestion for title}The majority of powerful and widely used LLMs are accessible % "white-box" \qin{May not be necessary to introduce this term} \peter{I also have seen people use "whitebox" to mean access to full internals, which seems to contradict definition here} settings via 
% through API calls, meaning that users only have access to output logits and not full model parameters. %without full access to model parameters. 
% \fb{Assuming access to output logits of a target policy $p_{\theta}$\footnote{Note that we use the terms target LM and target policy interchangeably.}, we define/instantiate? IPA as a neural network that is parameterized by $\phi$ and has shared vocabulary space as the target policy. In practice, we initialized IPA with a small language model in the same model family.}
% \sout{Hence, we assume "white-box" access for the target policy\footnote{Note that we use the terms target LM and target policy interchangeably.}\FB{this is the first time we use the term target policy. added footnote for now}, and define IPA as a neural network that is parameterized by $\phi$ and shares the same output space $p(\cdot|\textbf{y}_{<t})$ as the target policy. In practice, we initialized IPA with a small language model with shared vocabulary space as the target language model but fewer number of parameters.}

% We also define \textbf{adapted policy} $p_{\theta; \phi}$ as a product of experts combining the distributions of the target policy $p_{\theta}$ and the IPA $p_{\phi}$, formally 
% \FB{or over full Y with chain rule.}
% \begin{align} 
% p_{\theta; \phi} (\textbf{y}_{t}|\textbf{y}_{<t}) = \frac{1}{Z}  p_{\theta} (\textbf{y}_{t}|\textbf{y}_{<t}) p_{\phi}(\textbf{y}_{t}|\textbf{y}_{<t})
% \end{align}
% %\qin{This is our core equation. We should move it to where we describe the overall method, before "Initialization" }

% where $Z$ is a normalization factor to ensure valid probability distribution. Late fusion at distributional level enables us to tailor the behavior of the target policy without access to model parameter.

% \paragraph{Optimization} 
% \subsection{IPA Training with RL} \label{subsec:train-IPA}
% \FB{how about removing the subsection and go with paragraph.?}
\subsubsection{Training Adapter with RL}
% Our goal is to align the adapted policy with the user-specified objectives. The key idea is to achieve this alignment through RL but only updating the parameters of the adaptor policy. 

% Our goal is to align the adapted policy with the user-specified objectives.
% The key idea is to achieve this alignment through RL but only updating the parameters of the adaptor policy. 
We operationalize aligning the adapted policy with user-specified objectives through RL but only update the parameters of the adaptor policy.


Concretely, we leverage an RL algorithm $f_{\textnormal{RL}}$ from the family of online policy-based RL %\liwei{might be good to specify somewhere what "family of online policy-based RL" we refer to} \nouha{agree} \fb{it's mentioned in 2.3.2 and also later in this section after we talked about high-level stuff.}
to optimize the adapted policy $p_{\theta \leftarrow \phi}$ with respect to a given reward function $\mathcal{R}$. Notably, during the RL optimization, we freeze the parameters of the target policy $p_{\theta}$ and only update the parameters of the adaptor $p_{\phi}$, formally
% \begin{align}
%     \phi^\star = \arg\max \mathbb{E}_{\textbf{y}\sim p_{\theta; \phi}(\cdot | \textbf{x})}\mathcal{R}(\textbf{y})
% \end{align}
\begin{align*}
\phi^\star = f_{\textnormal{RL}} \: (p_{\theta \leftarrow \phi}, \mathcal{R}; \phi)
\end{align*}
\noindent Intuitively, the policy adaptor $p_\phi$ learns to fill in the gap \fb{what does fill in the gap mean here.} between the desired distribution with specified by the reward and the distribution returned by the base policy. \fb{Intuitively, the policy adapter learns to steer the distribution of the base policy towards the desired distribution with the specified reward.}
% Notice that
Our framework does not depend on a specific RL algorithm, but rather treats RL as a flexible plug-in optimization tool. As we will demonstrate later, \ipa proves to be effective when paired with any widely-used RL algorithm~\cite{Lu2022QuarkCT,Schulman2017ProximalPO} in the NLP field, and it can easily integrate any new RL algorithm innovations in the future.

For extremely large-scale language models like GPT-3, the forward pass is too costly to be used in the RL training loop. In such cases, we 
use an \textit{approximate base policy}, a smaller proxy model that approximates the target model's distribution, during the RL training.
\begin{definition}[approximate policy]
%The approximate policy is defined as a neural model with smaller size parameterized by $\hat{\theta}$ that approximates the distribution of the base policy and is used for adaptor training with RL, formally
The approximate policy is defined as a smaller-sized neural \fb{language?} model parameterized by $\hat{\theta}$ that approximates the distribution of the base policy and is used in replacement of the base policy in the RL-based adaptor training, formally
\vspace{-3mm}
\begin{align*}
\phi^\star = f_{\textnormal{RL}} \: (p_{\hat{\theta} \leftarrow \phi}, \mathcal{R}; \phi)
\end{align*}
\end{definition}
\vspace{-1mm}
%approximate the target policy $p_\theta$ with an \textbf{approximate policy} parameterized by $\hat{\theta}$ for RL optimization, %\fb{while still using the large-scale LM during decoding; }
%formally 
% \FB{we can skip the following equation. Doesn't add much info}
% \begin{align}
%     \phi^\star = \arg\max \mathbb{E}_{\textbf{y}\sim p_{\hat{\theta}; \phi}(\cdot | \textbf{x})}\mathcal{R}(\textbf{y})
% \end{align}
\nouha{I feel the approximate policy should be discussed before the policy adapter. }
\noindent In practice, we could use a smaller pre-trained language model from the same model family to be the approximate policy if it exhibits similar behavior in conditional generation $p(\textbf{y}|\textbf{x})$ with the base policy.
For instance, we use a off-the-shelf GPT2-XL as the approximate policy to tailor GPT-3 in the open-ended generation. Alternatively, we can use a distilled version of the base policy as the approximate policy, which can be obtained through sequence-level knowledge distillation \cite{kim2016sequencelevel}, $\hat{\theta} = \arg\max \mathbb{E}_{\textbf{y} \sim p_{\theta}(\cdot | \textbf{x})}\big[\log P_{\hat{\theta}}(\textbf{y})\big]$. For instance, we use a GPT2-XL fine-tuned with prompt-output pairs from GPT-3's generation as the approximate policy in the lexically constrained generation to tailor GPT-3.
% \paragraph{Decoding} 


\subsubsection{Applying Trained Adaptor to Guide Inference}

At inference time, we use the adapted policy $p_{\theta \leftarrow \phi}$ for decoding. At each time-step, we obtain the next-token distribution from the adapted policy $p_{\theta \leftarrow \phi} (\textbf{y}_{t}|\textbf{y}_{<t})$, which can then be used with any standard decoding algorithm (e.g., nucleus sampling).

%At inference time, we plug IPA trained with the approximate policy back into the target policy and generate with tailored policy $p_{\theta; \phi} (\textbf{y}_{t}|\textbf{y}_{<t})$.
%\\

%\fb{remember to explain ipa-, ipa*}
% \paragraph{Contribution}

% \begin{itemize}
%     \item Efficiency
%     \item Generalization
%     \item Modality
% \end{itemize}

==> tables/results_cot_acceptability.tex <==
% Please add the following required packages to your document preamble:
% \usepackage{multirow}
\begin{table}[]
\centering
\resizebox{0.49\textwidth}{!}{
\begin{tabular}{lccc}
\hline
\multicolumn{1}{l}{\multirow{2}{*}{\textbf{Models}}} & \textbf{Rationale} & \textbf{Task} & \textbf{Rationale} \\ 
\multicolumn{1}{c}{} & \textbf{Acceptability} & \textbf{Accuracy} \textbf{(\%)} & \textbf{Plausibility} \\
\hline
GPT-2$_\text{distill}$ & 0.34 & 53.73 & 0.59 \\ %0.29 & 53.73 \\
GPT-3 & 0.41 & 78.38 & 0.72 \\ \hline
IPA (GPT-2$_\text{distill}$) & 0.42 & 52.74 & 0.58 \\ %0.34 & 54.38 \\
IPA (GPT-3) & \textbf{0.5} & 78.05 & \textbf{0.73} \\
\hline
\end{tabular}
}
\caption{Results for \textit{self-rationalization} in question-answering. The reported results are on the validation set of \csqa.}
\label{tab:csqa_rationalization}
\end{table}

==> tables/results_open_domain_human.tex <==

\begin{table*}[t]
\centering
\footnotesize
\renewcommand{\arraystretch}{1.5}
\setlength\tabcolsep{3pt}
\begin{tabular}{l|l|ccclccclccc}
\midrule
\multirow{2}{*}{\textbf{Method}} & \multirow{2}{*}{\textbf{Baseline}} & \multicolumn{3}{c}{\textbf{More Fluent}} &  & \multicolumn{3}{c}{\textbf{More Coherent}} &  & \multicolumn{3}{c}{\textbf{Better Overall}} \\ \cline{3-5} \cline{7-9} \cline{11-13} 
                                 &                                    & method          & tie     & baseline     &  & method           & tie      & baseline     &  & method           & tie      & baseline      \\ \hline
\multirow{7}{*}{IPA- (GPT2-XL)}             & greedy                             & \textbf{49}     & 6       & 31           &  & \textbf{56}      & 7        & 23           &  & \textbf{44}      & 7        & 29            \\
                                 % & truncation                         & \textbf{56}     & 4       & 19           &  & \textbf{50}      & 6        & 24           &  & \textbf{55}      & 7        & 25            \\
                                 & top-k (k=50)                       & \textbf{48}     & 6       & 28           &  & \textbf{44}      & 4        & 35           &  & \textbf{51}      & 7        & 31            \\
                                 & top-p (p=0.95)                     & \textbf{48}     & 1       & 34           &  & \textbf{47}      & 4        & 37           &  & \textbf{59}      & 1        & 23            \\
                                 & typical ($\tau$=0.95)                   & \textbf{43}     & 5       & 38           &  & \textbf{54}      & 2        & 36           &  & \textbf{54}      & 3        & 34            \\
                                 & SimCTG                             & \textbf{53}     & 5       & 27           &  & \textbf{56}      & 3        & 30           &  & \textbf{53}      & 7        & 27            \\
                                 & Contrastive                        & \textbf{42}     & 9       & 32           &  & \textbf{55}      & 3        & 33           &  & \textbf{53}      & 3        & 32            \\ \hline
\ipa- (GPT-3)                             & \multirow{2}{*}{GPT-3}             &           \textbf{46}      &      3   &        35      &  &      35            &     5     &      \textbf{44}        &  &         \textbf{45}         &      4    &  34             \\
\ipastar(GPT-3)                            &                              &     \textbf{44}       &   4   &         37     &  &     \textbf{36}             &     8     &        32      &  &          \textbf{43}        &    3      &        34       \\ \midrule
\end{tabular}
\caption{Pairwise human evaluation for \textit{open-domain generations} on XSum. \liwei{this table feels a little sparse. if time permit, could consider turn this into plots such as the ones reported in dexpert}\jaehun{agreed, a minor thing but we could benefit from more figures / plots in replace of tables overall}\fb{plots sound better for this table. Will give it a shot soon}}
\label{tab:open-domain-human}
\end{table*}
